Tractability and Decompositions of Global Cost Functions

Enforcing local consistencies in cost function networks is performed by applying so-called Equivalent Preserving Transformations (EPTs) to the cost functions. As EPTs transform the cost functions, they may break the property that was making local consistency enforcement tractable on a global cost function. A global cost function is called tractable projection-safe when applying an EPT to it is tractable and does not break the tractability property. In this paper, we prove that depending on the size r of the smallest scopes used for performing EPTs, the tractability of global cost functions can be preserved (r = 0) or destroyed (r > 1). When r = 1, the answer is indefinite. We show that on a large family of cost functions, EPTs can be computed via dynamic programming-based algorithms, leading to tractable projection-safety. We also show that when a global cost function can be decomposed into a Berge acyclic network of bounded arity cost functions, soft local consistencies such as soft Directed or Virtual Arc Consistency can directly emulate dynamic programming. These different approaches to decomposable cost functions are then embedded in a solver for extensive experiments that confirm the feasibility and efficiency of our proposal.

==> related.tex <==
% Currently edited by: 

%\subsection{Related Work}\label{related}
%Global constraints define one of the key elements that participated to the success of CSP and Constraint programming. Starting from
%\CiteInLine{JLL1978}, many global constraints have been proposed and studied. To help categorize global constraints, Beldiceanu \etal \citeyear{NB2000,NMT2004,BCR2005} further develop a representation scheme for global constraints using a graph-based and an automaton approach. Various techniques have been applied to enforce local consistency on global constraints.  For example, matching theory has been used for enforcing Arc Consistency on the  \gc{AllDifferent} constraint~\cite{JCR1994,Pug1998} introduced in~\cite{JLL1978}, flow theory has been applied to \gc{GCC} \cite{JCR1996} and \gc{Same}~\cite{NIS2004}. Dynamic programming approaches have been suggested for \gc{Regular} \cite{GP2004} and \gc{Grammar} \cite{KS2010}. Through modeling by \gc{Regular}~\cite{GP2004} and \gc{Grammar}~\cite{KS2010}, it is possible to define simple enforcement algorithms for \gc{Among} and \gc{Sequence}~\cite{WGLA2006}, line sweeping algorithms have also been applied for the \gc{Maximum} and \gc{Minimum} constraints~\cite{NB2001}. Notice that not all consistency enforcing algorithms are tractable.  \CiteInLine{CEBT2004a} investigate and give detailed results on tractability of global constraint enforcement.  Similar techniques can also be applied to soft global constraints. For example, van Hoeve \etal \citeyear{WGL2006} develop a framework for enforcing  classical arc consistency on soft global constraints representable by flow networks, whose computation is polynomial in the size of networks.

%Based on the work of van Hoeve~\etal~\citeyear{WGL2006}, \CiteInLine{LL2009,LL2012asa} have introduced a framework to enforce \emph{soft} arc consistencies on corresponding global cost functions using flow algorithms, later extended in~\citeyear{LS2011,LS2012,lee2014} by using linear programming. In this paper, we extend the area of tractable global cost function by instead using dynamic programming or an emulation of dynamic programming based on soft arc consistencies.
% On the other hand, to efficiently remove more search space during
% WCSPs solving, various consistency notions have been
% developed. Examples are NC* \cite{JT2004_AC}, BAC$^\varnothing$
% \cite{MCT2009}, strong $\varnothing$IC\cite{LL2012asa}, (G)AC*
% \cite{JT2004_AC,LL2012asa}, FD(G)AC* \cite{JT2003_FDAC,LL2012asa}, and
% (weak) ED(G)AC* \cite{GHZL2005,LL2012asa}. Stronger consistency
% notions, namely OSAC and VAC \shortcite{Cooper2010}, are also defined,
% but enforcement requires a relaxation of the cost valuation structure
% $V(\top)$ to rational numbers.
%, and current implementations are efficient only on binary WCSPs
% For ternary cost functions, AC, FDAC and EDAC are introduced
% \shortcite{MST2008}.  Cooper \citeyear{MC2005} incorporates the
% concept of $k$-consistency into WCSPs to form \emph{complete
% $k$-consistency}. However, most enforcement becomes impractical if the
% arity of the cost functions increases. To make the consistency
% enforcement practical for high-arity cost functions,
% \CiteInLine{LL2012asa} have developed a framework that integrates
% global cost functions into WCSPs
% and made the enforcement become polynomial.
